Regularizing Black-box Models for Improved Interpretability (HILL 2019 Version)

Most of the work on interpretable machine learning has focused on designing either inherently interpretable models, which typically trade-off accuracy for interpretability, or post-hoc explanation systems, which lack guarantees about their explanation quality. We propose an alternative to these approaches by directly regularizing a black-box model for interpretability at training time. Our approach explicitly connects three key aspects of interpretable machine learning: (i) the model's innate explainability, (ii) the explanation system used at test time, and (iii) the metrics that measure explanation quality. Our regularization results in substantial improvement in terms of the explanation fidelity and stability metrics across a range of datasets and black-box explanation systems while slightly improving accuracy. Further, if the resulting model is still not sufficiently interpretable, the weight of the regularization term can be adjusted to achieve the desired trade-off between accuracy and interpretability. Finally, we justify theoretically that the benefits of explanation-based regularization generalize to unseen points.

==> figures/expo-algorithms-old.tex <==

\begin{figure}[t]
\begin{minipage}[t]{0.48\textwidth}
\begin{algorithm}[H]
    \caption{Learning with \name}
    \label{alg:expo}
    \begin{algorithmic}[1]
    \small\vspace{2pt}
    \INPUT $\Dc$ -- dataset, $\gamma$ -- regularization coefficient,\\
           $N_x^\mathrm{reg}$ -- neighborhood sampling function,\\
           $T$ -- number of optimization epochs.
    \STATE Initialize model $f$ with parameters $\theta_0$.
    \FOR{$t$ in $0 \dots T$}
        \FOR{each of mini-batch $\Bc$ in $\Dc$}
            \FOR{each point $x_i$ in $\Bc$}
                \STATE Regularizer: $r(\theta, x_i) = \Rc(f_{\theta}, N_{x_i}^\mathrm{reg})$\\
                       (compute using Algorithm \ref{alg:expo-fidelity-reg} or \ref{alg:expo-stability-reg}).
            \ENDFOR
            \STATE Construct loss:
            \vspace{-1ex}
            \begin{equation*}
                L(\theta) := \frac{1}{|\Bc|} \sum_{x_i \in \Bc} \Lc(\theta, x_i) + \gamma r(\theta, x_i).
            \end{equation*}
            \vspace{-2ex}
            \STATE Update the model:
            \begin{equation*}
                \theta_{t+1} \leftarrow \mathrm{update}(\theta_t, \nabla L(\theta_t))
            \end{equation*}
        \ENDFOR
    \ENDFOR
    \OUTPUT Learned model, $f_{\theta_T}$.
    \vspace{5.5pt}
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\quad
\begin{minipage}[t]{0.48\textwidth}
\begin{algorithm}[H]
    \caption{Neighborhood-fidelity regularizer}
    \label{alg:expo-fidelity-reg}
    \begin{algorithmic}[1]
    \small\vspace{2pt}
    \INPUT $f_\theta$, $x$, $N_x^\mathrm{reg}$, $m$
    \STATE Sample points: $x'_1, \dots, x'_m \sim N_x^\mathrm{reg}$
    \STATE Compute predictions:
    \begin{equation*}
        \hat y_j(\theta) = f_\theta(x'_j) \text{ for } j = 1, \dots, m
    \end{equation*}
    \STATE Produce a local linear explanation:
    \begin{equation*}
        \beta_x(\theta) = \argmin_\beta \sum_{j=1}^m (\hat y_j(\theta) - \beta^\top x'_j)^2
    \end{equation*}
    \OUTPUT $\frac{1}{m}\sum_{j=1}^m (\hat y_f(\theta) - \beta_x(\theta)^\top x'_j)^2$
    \end{algorithmic}
\end{algorithm}
\vspace{-5.7ex}
\begin{algorithm}[H]
    \caption{Neighborhood-stability regularizer}
    \label{alg:expo-stability-reg}
    \begin{algorithmic}[1]
    \small\vspace{2pt}
    \INPUT $f_\theta$, $x$, $N_x^\mathrm{reg}$, $m$
    \STATE Sample points: $x'_1, \dots, x'_m \sim N_x^\mathrm{reg}$
    \STATE Compute predictions:
    \begin{equation*}
        \hat y_j(\theta) = f_\theta(x'_j), \text{ for } j = 1, \dots, m
    \end{equation*}
    \OUTPUT $\frac{1}{m}\sum_{j=1}^m (\hat y_j(\theta) - f(x))^2$
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\end{figure}


==> sections/scratch.tex <==
\begin{figure}[t]
    \centering
    \floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,center},capbesidewidth=0.4\textwidth}}]{figure}[\FBwidth]
    {\caption{%
    The effects of our regularizer on a model predicting Bob's credit rating.
    The abrupt kinks in the unregularized model make the local linear approximations both less faithful to the model and less stable to small perturbations.  
    The regularized model is much smoother and therefore easier to explain.  
    Also observe that, when over-regularized, we can force the learned function to be essentially linear.}%
    \label{fig:toy}}
    {\includegraphics[width=0.5\textwidth]{figures/ToyExample.png}}
\end{figure}
